VE: Modeling Multivariate Time Series Correlation with Variate Embedding

Multivariate time series forecasting relies on accurately capturing the correlations among variates. Current channel-independent (CI) models and models with a CI final projection layer are unable to capture these dependencies. In this paper, we present the variate embedding (VE) pipeline, which learns a unique and consistent embedding for each variate and combines it with Mixture of Experts (MoE) and Low-Rank Adaptation (LoRA) techniques to enhance forecasting performance while controlling parameter size. The VE pipeline can be integrated into any model with a CI final projection layer to improve multivariate forecasting. The learned VE effectively groups variates with similar temporal patterns and separates those with low correlations. The effectiveness of the VE pipeline is demonstrated through experiments on four widely-used datasets. The code is available at: https://github.com/swang-song/VE.

==> Chapters/chapter1.tex <==

\appendix

\subsection{Related work: traditional statistical methods and basic deep neural network architectures}\label{app:related_work}
% \subsection{Related work: traditional statistical methods and basic deep neural network architectures}
\begin{itemize}
    \item Statistical methods, such as autoregressive integrated moving average (ARIMA), perform poorly due to their predefined fixed patterns, which are incapable of handling real-world data that exhibit complex patterns. These methods have simple architectures with low modeling capability to handle multivariate time series, and suffer from low generalizability (requiring a new model to be retrained for each shifted series in each channel) \cite{box2015time}.
    \item Deep neural networks have become popular due to their strong modeling capacity and data-driven nature, which allows them to adapt to any latent data patterns. 
    Recurrent neural networks (RNNs)-based models \cite{wen2017multi, lai2018modeling, salinas2020deepar} rely on recurrence to capture temporal dependencies, while convolutional neural networks (CNNs)-based models \cite{vanoord2016wavenet, bai2018empirical, liu2022scinet} use convolution to model local temporal patterns. 
    However, both struggle to handle long-term dependencies. 
    Transformer-based models, due to their exceptional capability of handling long-term dependencies with the attention mechanism, have outperformed RNNs and CNNs in long-term time series forecasting \cite{liu2023itransformer, ilbert2024unlocking}. 
\end{itemize}

% \subsection{Experimental Details}
% \subsubsection{Dataset details}
\subsection{Dataset details}\label{app:dataset_details}
The details of each dataset are:
\begin{itemize} 
    \item \textbf{ETTh1} and \textbf{ETTh2}: These are two electricity transformer temperature datasets, each containing one oil temperature and six load features recorded on an hourly basis in two different countries. 
    The data spans from 2016-07-01 to 2018-06-26. 
    \item \textbf{ECL}: This dataset collects the hourly electricity consumption load of 321 clients in kilowatt-hours (kWh) from 2012-01-01 to 2014-12-31. 
    \item \textbf{Weather}: This dataset includes 21 weather indicators, such as air temperature, wind velocity, and rain, recorded every 10 minutes from 2020-01-01 to 2020-12-31. 
\end{itemize}
The characteristics of these datasets are listed in Table \ref{tab:datasets_statistics}.

\begin{table}[ht]
    \centering
    \caption{Datasets statistics}
    \label{tab:datasets_statistics}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{@{}cccccc@{}}
    \toprule
    Datasets                     & Variates & Timesteps & Granularity & Start time & end time   \\ \midrule
    \multicolumn{1}{c|}{ETTh1}   & 7        & 17420     & 1hour       & 01/07/2016 & 26/06/2018 \\
    \multicolumn{1}{c|}{ETTh2}   & 7        & 17420     & 1hour       & 01/07/2016 & 26/06/2018 \\
    \multicolumn{1}{c|}{ECL}     & 321      & 26304     & 1hour       & 01/01/2012 & 31/12/2014 \\
    \multicolumn{1}{c|}{Weather} & 21       & 52696     & 10min       & 01/01/2020 & 31/12/2020 \\ \bottomrule
    \end{tabular}%
    }
\end{table}

\subsection{Implementation Details}\label{app:implementation_details}
\textbf{Implementation details}.
There are two hyperparameter in our proposed VE pipeline:
the variate embedding dimension
$k$, and the parameter size expansion ratio
$p$.
we conduct a grid search over 
$k$ in \{2, 4, 8, 16, 32, 64, 128\}, and 
$p$ in \{0.25, 1, 4\}.
For the hyperparameters of the baseline models, we use the default settings in their official code unless otherwise stated. 
The training epochs of PatchTST \cite{nie2022time} is reduced from 100 to 10 to free up time for more expentiments.
We utilize RevIN \cite{kim2021reversible} to boost the performance of all models. The data splits for training, validation, and testing adhere to standard practices in the field: a 6:2:2 ratio for the ETT datasets and a 7:1:2 ratio for the other datasets.
% We employ the Time Series library (TSlib) \cite{wu2022timesnet} to ensure consistent evaluation pipelines and data splits across experiments. 
All experiments are conducted on a single NVIDIA GeForce RTX 4060 Ti 8GB GPU. 
We run each experiment three times using random seeds 2021, 2022, and 2023, as used in PatchTST \cite{nie2022time}, and report the mean values.


\subsection{Multivariate forecasting for each dataset: standard deviation values}\label{app:std_results}
Table \ref{tab:std_all} reports the standard deviation values for Table \ref{tab:mse_all} in the main text.

\begin{table*}[!ht]
    \centering
    \caption{The standard deviation values for the comparison results between baselines and proposed VE on ETTh1, ETTh2, ECL and Weather with prediction horizon 
    $H \in \{92, 192\}$.}
    \label{tab:std_all}
    \begin{tabular}{@{}cccccccccccc@{}}
    \toprule
    \multicolumn{2}{c}{Method}                                               & FITS  & +VE                        & Linear & +VE                        & DLinear & +VE                        & iTransformer & +VE                        & PatchTST & +VE   \\ \midrule
    \multicolumn{1}{c|}{\multirow{2}{*}{ETTh1}}   & \multicolumn{1}{c|}{96}  & 0.000 & \multicolumn{1}{c|}{0.000} & 0.000  & \multicolumn{1}{c|}{0.000} & 0.005   & \multicolumn{1}{c|}{0.001} & 0.000        & \multicolumn{1}{c|}{0.000} & 0.005    & 0.002 \\
    \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{192} & 0.005 & \multicolumn{1}{c|}{0.001} & 0.000  & \multicolumn{1}{c|}{0.001} & 0.001   & \multicolumn{1}{c|}{0.001} & 0.005        & \multicolumn{1}{c|}{0.001} & 0.006    & 0.001 \\ \midrule
    \multicolumn{1}{c|}{\multirow{2}{*}{ETTh2}}   & \multicolumn{1}{c|}{96}  & 0.000 & \multicolumn{1}{c|}{0.000} & 0.001  & \multicolumn{1}{c|}{0.001} & 0.005   & \multicolumn{1}{c|}{0.001} & 0.001        & \multicolumn{1}{c|}{0.001} & 0.001    & 0.001 \\
    \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{192} & 0.000 & \multicolumn{1}{c|}{0.001} & 0.001  & \multicolumn{1}{c|}{0.001} & 0.007   & \multicolumn{1}{c|}{0.001} & 0.001        & \multicolumn{1}{c|}{0.001} & 0.003    & 0.001 \\ \midrule
    \multicolumn{1}{c|}{\multirow{2}{*}{ECL}}     & \multicolumn{1}{c|}{96}  & 0.000 & \multicolumn{1}{c|}{0.000} & 0.000  & \multicolumn{1}{c|}{0.000} & 0.000   & \multicolumn{1}{c|}{0.000} & 0.000        & \multicolumn{1}{c|}{0.000} & -        & -     \\
    \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{192} & 0.000 & \multicolumn{1}{c|}{0.000} & 0.000  & \multicolumn{1}{c|}{0.000} & 0.000   & \multicolumn{1}{c|}{0.000} & 0.000        & \multicolumn{1}{c|}{0.000} & -        & -     \\ \midrule
    \multicolumn{1}{c|}{\multirow{2}{*}{Weather}} & \multicolumn{1}{c|}{96}  & 0.000 & \multicolumn{1}{c|}{0.000} & 0.000  & \multicolumn{1}{c|}{0.000} & 0.000   & \multicolumn{1}{c|}{0.001} & 0.005        & \multicolumn{1}{c|}{0.002} & 0.002    & 0.001 \\
    \multicolumn{1}{c|}{}                         & \multicolumn{1}{c|}{192} & 0.000 & \multicolumn{1}{c|}{0.000} & 0.000  & \multicolumn{1}{c|}{0.000} & 0.000   & \multicolumn{1}{c|}{0.001} & 0.001        & \multicolumn{1}{c|}{0.001} & 0.001    & 0.001 \\ \bottomrule
    \end{tabular}
\end{table*}







\begin{figure}[!t]
    \centering
    \includegraphics[width=0.8\linewidth]{images/351_to_355_weights.pdf}
    \caption{Visualization of the weights ($softmax(VE)$) of FITS($H=96, k=8$) to the linear experts for variates from 351 to 355.}
    \label{fig::softmax_weights_351_to_355}
\end{figure}

\subsection{Visualization of VE softmax weights}\label{app:visual_softmax_weights}
The softmax weights for variates 351 to 355 are depicted in Fig. \ref{fig::softmax_weights_351_to_355}. 
Variates 331, 332, and 333 show a strong emphasis on experts 0 and 1, indicating that these variates are closely related and thus share similar embedding weights. 
On the other hand, variate 354 has the highest weights assigned to expert 5, while variate 355 shows much more stronger association with expert 6 than other variates. These results are consistent with the observations made in Fig. \ref{fig::VE_cos_similarity} (middle and right panels), reinforcing the idea that the variates with similar temporal patterns have high softmax weights for the same experts, while variates with different patterns focus on different experts.


% The softmax weights of these five variates are visualized in Fig. \ref{fig::softmax_weights_351_to_355}.
% It can be seen that variates 331, 332, 333 learn similar weights with an emphasis to expert 0 and 1, while variate 354 has the highest weights on expert 5 and variate 355 has the highest weights on expert 6.
% This shows consistent results with the observations in Fig. \ref{fig::VE_cos_similarity} (middle and right panels).








\subsection{Hyperparameter sensitivity}\label{app:param_sensitivity}


We explore the sensitivity of the variate embedding dimension ($k$) and parameter size expansion factor ($p$) on the all datasets for all models.
The results of the hyperparameter sensitivity on ETTh1, ETTh2, ECL and Weather for prediction length 192 are listed in Table \ref{tab:paramsensitivity_ETTh1}, \ref{tab:paramsensitivity_ETTh2}, \ref{tab:paramsensitivity_ECL} and \ref{tab:paramsensitivity}

It can be seen that the optimal parameter settings are highly dataset-specific, with different datasets showing preferences for distinct hyperparameter values for each model. 

% Additional sensitivity studies on ETTh1, ETTh2, and Weather datasets can be found in the Table \ref{tab:paramsensitivity_ETTh1}, \ref{tab:paramsensitivity_ETTh2} and \ref{tab:paramsensitivity}.



% \subsection{Hyperparameter sensitivity}.
% We explore the sensitivity of the variate embedding dimension ($k$) and parameter size expansion factor ($p$) on the ECL dataset, with the results presented in Table \ref{tab:Abalation}. 
% The findings indicate that maintaining the model size at the original level ($p=1$) generally yields performance comparable to models with four times the parameters ($p=4$). 
% For models like iTransformer and FITS, which involve processing inputs to obtain high-level representations, larger embedding dimensions ($k=8$) are beneficial. Conversely, linear models that do not explore high-level representations tend to favor smaller embedding dimensions ($k=2$).

% It is important to note that the optimal parameter settings are highly dataset-specific, with different datasets showing preferences for distinct hyperparameter values for each model. Additional sensitivity studies on ETTh1, ETTh2, and Weather datasets can be found in the Table \ref{tab:paramsensitivity_ETTh1}, \ref{tab:paramsensitivity_ETTh2} and \ref{tab:paramsensitivity}.










\begin{table*}[!ht]
    \centering
    \caption{Hyperparameter sensitivity analysis of the VE pipeline with respect to the variate embedding dimension ($k$) and parameter size expansion factor ($p$) on the ETTh1 dataset. The best results within each parameter size level are shaded, and the absolute \textbf{best result} for each model is highlighted in \textbf{bold}.}
    \label{tab:paramsensitivity_ETTh1}
    \begin{tabular}{@{}cclllllll@{}}
    \toprule
                                                        &                           & \multicolumn{7}{c}{$k$}                                                                                                                                                                                                                                                           \\ \cmidrule(l){3-9} 
    \multirow{-2}{*}{Method}                            & \multirow{-2}{*}{$p$}       & \multicolumn{1}{c}{2}                      & \multicolumn{1}{c}{4} & \multicolumn{1}{c}{8}                      & \multicolumn{1}{c}{16}                     & \multicolumn{1}{c}{32}                    & \multicolumn{1}{c}{64}                     & \multicolumn{1}{c}{128} \\ \midrule
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{0.25} & \cellcolor[HTML]{F2F2F2}0.5759137          & 0.6025965             & 0.6193596                                  & 0.6672822                                  &                                           &                                            &                         \\
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{1}    & \cellcolor[HTML]{F2F2F2}0.4527064          & 0.4561656             & 0.4556148                                  & 0.4654581                                  & 0.4759384                                 & 0.5462764                                  &                         \\
    \multicolumn{1}{c|}{\multirow{-3}{*}{iTransformer}} & \multicolumn{1}{c|}{4}    & 0.4370797                                  & 0.4377286             & \cellcolor[HTML]{F2F2F2}\textbf{0.4368649} & 0.437161                                   & 0.4393856                                 & 0.4414116                                  & 0.4429454               \\ \midrule
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{0.25} & \cellcolor[HTML]{F2F2F2}0.4151344          & 0.4201289             & 0.4203557                                  & 0.4162619                                  &                                           &                                            &                         \\
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{1}    & \cellcolor[HTML]{F2F2F2}\textbf{0.4062881} & 0.4090861             & 0.4222339                                  & 0.4101511                                  & 0.4129601                                 & 0.4159569                                  &                         \\
    \multicolumn{1}{c|}{\multirow{-3}{*}{Dlinear}}      & \multicolumn{1}{c|}{4}    & \cellcolor[HTML]{F2F2F2}0.4081776          & 0.4083269             & 0.4100214                                  & 0.4125096                                  & 0.4089666                                 & 0.4109049                                  & 0.4088479               \\ \midrule
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{0.25} & \cellcolor[HTML]{F2F2F2}0.4746067          & 0.4898597             & 0.5236394                                  & 0.6261807                                  &                                           &                                            &                         \\
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{1}    & 0.4307631                                  & 0.4290519             & \cellcolor[HTML]{F2F2F2}0.4232234          & 0.4243045                                  & 0.4332948                                 & 0.4753141                                  &                         \\
    \multicolumn{1}{c|}{\multirow{-3}{*}{Linear}}       & \multicolumn{1}{c|}{4}    & 0.4173298                                  & 0.4246842             & 0.4233281                                  & 0.4179523                                  & \cellcolor[HTML]{F2F2F2}\textbf{0.413765} & 0.4155265                                  & 0.4195332               \\ \midrule
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{0.25} & 0.4404356                                  & 0.4428441             & \cellcolor[HTML]{F2F2F2}0.4402694          & 0.4569152                                  & 0.4521996                                 &                                            &                         \\
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{1}    & 0.4361777                                  & 0.4335845             & 0.4421907                                  & \cellcolor[HTML]{F2F2F2}\textbf{0.4281024} & 0.4343016                                 & 0.4333888                                  & 0.4375243               \\
    \multicolumn{1}{c|}{\multirow{-3}{*}{PatchTST}}     & \multicolumn{1}{c|}{4}    & 0.447887                                   & 0.4444195             & 0.4365204                                  & 0.4316048                                  & \cellcolor[HTML]{F2F2F2}0.4294316         & 0.4295166                                  & 0.4394555               \\ \midrule
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{0.25} & 0.4202258                                  & 0.4148696             & 0.4153076                                  & \cellcolor[HTML]{F2F2F2}0.4143093          &                                           &                                            &                         \\
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{1}    & 0.4130148                                  & 0.4093615             & \cellcolor[HTML]{F2F2F2}0.4051334          & 0.4071268                                  & 0.4095037                                 & 0.4076311                                  &                         \\
    \multicolumn{1}{c|}{\multirow{-3}{*}{FITS}}         & \multicolumn{1}{c|}{4}    & 0.4177962                                  & 0.4103759             & 0.4067034                                  & 0.405706                                   & 0.4055257                                 & \cellcolor[HTML]{F2F2F2}\textbf{0.4041664} & 0.4045437               \\ \bottomrule
    \end{tabular}
\end{table*}









\begin{table*}[!ht]
    \centering
    \caption{Hyperparameter sensitivity analysis of the VE pipeline with respect to the variate embedding dimension ($k$) and parameter size expansion factor ($p$) on the ETTH2 dataset. The best results within each parameter size level are shaded, and the absolute \textbf{best result} for each model is highlighted in \textbf{bold}.}
    \label{tab:paramsensitivity_ETTh2}
    \begin{tabular}{@{}cclllllll@{}}
    \toprule
                                                        &                           & \multicolumn{7}{c}{$k$}                                                                                                                                                                                                                                                             \\ \cmidrule(l){3-9} 
    \multirow{-2}{*}{Method}                            & \multirow{-2}{*}{$p$}       & \multicolumn{1}{c}{2}                      & \multicolumn{1}{c}{4}             & \multicolumn{1}{c}{8}             & \multicolumn{1}{c}{16}                     & \multicolumn{1}{c}{32}                    & \multicolumn{1}{c}{64} & \multicolumn{1}{c}{128}                    \\ \midrule
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{0.25} & \cellcolor[HTML]{F2F2F2}0.414456           & 0.4192579                         & 0.419987                          & 0.4191134                                  &                                           &                        &                                            \\
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{1}    & 0.3874659                                  & \cellcolor[HTML]{F2F2F2}0.3852195 & 0.3874141                         & 0.3917341                                  & 0.3953916                                 & 0.4002145              &                                            \\
    \multicolumn{1}{c|}{\multirow{-3}{*}{iTransformer}} & \multicolumn{1}{c|}{4}    & 0.3797458                                  & 0.3798732                         & 0.3808539                         & 0.3803457                                  & \cellcolor[HTML]{F2F2F2}\textbf{0.377773} & 0.3805791              & 0.3838764                                  \\ \midrule
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{0.25} & 0.3396295                                  & 0.3384397                         & \cellcolor[HTML]{F2F2F2}0.3320681 & 0.3375999                                  &                                           &                        &                                            \\
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{1}    & 0.334612                                   & \cellcolor[HTML]{F2F2F2}0.3332178 & 0.338977                          & 0.337763                                   & 0.3355195                                 & 0.3354599              &                                            \\
    \multicolumn{1}{c|}{\multirow{-3}{*}{Dlinear}}      & \multicolumn{1}{c|}{4}    & \cellcolor[HTML]{F2F2F2}\textbf{0.3311656} & 0.3542754                         & 0.3466274                         & 0.3410067                                  & 0.3389088                                 & 0.3377589              & 0.3343827                                  \\ \midrule
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{0.25} & 0.3654841                                  & \cellcolor[HTML]{F2F2F2}0.3638662 & 0.3664166                         & 0.3800778                                  &                                           &                        &                                            \\
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{1}    & 0.3513539                                  & 0.344813                          & 0.3424248                         & \cellcolor[HTML]{F2F2F2}0.3420352          & 0.3455624                                 & 0.3574789              &                                            \\
    \multicolumn{1}{c|}{\multirow{-3}{*}{Linear}}       & \multicolumn{1}{c|}{4}    & 0.3461033                                  & 0.3458244                         & 0.3378494                         & \cellcolor[HTML]{F2F2F2}\textbf{0.3328552} & 0.3358812                                 & 0.3395165              & 0.3405563                                  \\ \midrule
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{0.25} & \cellcolor[HTML]{F2F2F2}0.3664075          & 0.3674269                         & 0.3704121                         & 0.3731442                                  & 0.3794572                                 &                        &                                            \\
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{1}    & 0.372417                                   & 0.3662166                         & 0.3731748                         & \cellcolor[HTML]{F2F2F2}0.3620954          & 0.363443                                  & 0.365167               & 0.3666856                                  \\
    \multicolumn{1}{c|}{\multirow{-3}{*}{PatchTST}}     & \multicolumn{1}{c|}{4}    & 0.3702272                                  & 0.3660711                         & 0.3679468                         & 0.3642895                                  & 0.3693766                                 & 0.3592695              & \cellcolor[HTML]{F2F2F2}\textbf{0.3578018} \\ \midrule
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{0.25} & 0.3339219                                  & 0.339437                          & \cellcolor[HTML]{F2F2F2}0.3320387 & 0.3336499                                  &                                           &                        &                                            \\
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{1}    & 0.3326842                                  & 0.3351202                         & 0.3304985                         & 0.3287979                                  & \cellcolor[HTML]{F2F2F2}0.3283068         & 0.3290774              &                                            \\
    \multicolumn{1}{c|}{\multirow{-3}{*}{FITS}}         & \multicolumn{1}{c|}{4}    & 0.3346798                                  & 0.3335502                         & 0.3299259                         & 0.3279871                                  & 0.3284978                                 & 0.3277869              & \cellcolor[HTML]{F2F2F2}\textbf{0.3269419} \\ \bottomrule
    \end{tabular}
\end{table*}






\begin{table*}[htb]
    \centering
    \caption{Hyperparameter sensitivity analysis of the VE pipeline with respect to the variate embedding dimension ($k$) and parameter size expansion factor ($p$) on the ECL dataset. The best results within each parameter size level are shaded, and the absolute \textbf{best result} for each model is highlighted in \textbf{bold}.}
    % \caption{Hyperparameter sensitivity analysis of the VE pipeline with respect to the variate embedding dimension ($k$) and parameter size expansion factor ($p$) on the ECL dataset. The best results within each parameter size level are shaded, and the absolute \textbf{best result} for each model is highlighted in \textbf{bold}.}
    \label{tab:paramsensitivity_ECL}
    \begin{tabular}{@{}cclllllll@{}}
    \toprule
                                                        &                           & \multicolumn{7}{c}{$k$}                                                                                                                                                                                                \\ \cmidrule(l){3-9} 
    \multirow{-2}{*}{Method}                            & \multirow{-2}{*}{$p$}       & \multicolumn{1}{c}{2}                      & \multicolumn{1}{c}{4} & \multicolumn{1}{c}{8}                      & \multicolumn{1}{c}{16} & \multicolumn{1}{c}{32} & \multicolumn{1}{c}{64} & \multicolumn{1}{c}{128} \\ \midrule
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{0.25} & \cellcolor[HTML]{F2F2F2}0.1809065          & 0.1854654             & 0.1927616                                  & 0.2006371              & 0.2114202              &                        &                         \\
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{1}    & \cellcolor[HTML]{F2F2F2}0.1609274          & 0.1619309             & 0.1630106                                  & 0.1640473              &                        &                        &                         \\
    \multicolumn{1}{c|}{\multirow{-3}{*}{iTransformer}} & \multicolumn{1}{c|}{4}    & 0.1581553                                  & 0.1571849             & \cellcolor[HTML]{F2F2F2}\textbf{0.1571855} & 0.1576903              & 0.1593817              & 0.1603102              & 0.1612906               \\ \midrule
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{0.25} & \cellcolor[HTML]{F2F2F2}0.1617287          & 0.1647222             & 0.1728343                                  & 0.1902601              &                        &                        &                         \\
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{1}    & \cellcolor[HTML]{F2F2F2}0.1511226          & 0.152687              & 0.1534423                                  & 0.1548727              & 0.1570784              & 0.1638301              &                         \\
    \multicolumn{1}{c|}{\multirow{-3}{*}{Dlinear}}      & \multicolumn{1}{c|}{4}    & \cellcolor[HTML]{F2F2F2}\textbf{0.1492961} & 0.150592              & 0.1507927                                  & 0.1510172              & 0.15126                & 0.1519248              & 0.1527796               \\ \midrule
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{0.25} & \cellcolor[HTML]{F2F2F2}0.2286057          & 0.2387695             & 0.2610307                                  & 0.3578889              &                        &                        &                         \\
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{1}    & \cellcolor[HTML]{F2F2F2}0.1707352          & 0.1730516             & 0.1734239                                  & 0.1768471              & 0.1896042              & 0.2226846              &                         \\
    \multicolumn{1}{c|}{\multirow{-3}{*}{Linear}}       & \multicolumn{1}{c|}{4}    & \cellcolor[HTML]{F2F2F2}\textbf{0.1584287} & 0.1587195             & 0.158627                                   & 0.1593248              & 0.1611207              & 0.1651422              & 0.1723562               \\ \midrule
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{0.25} & \cellcolor[HTML]{F2F2F2}0.1510328          & 0.1517532             & 0.1516034                                  & 0.1531377              & 0.1541373              &                        &                         \\
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{1}    & 0.1495172                                  & 0.1486223             & \cellcolor[HTML]{F2F2F2}0.1479547          & 0.1487291              & 0.1492981              & 0.1495262              & 0.1497324               \\
    \multicolumn{1}{c|}{\multirow{-3}{*}{FITS}}         & \multicolumn{1}{c|}{4}    & 0.1498906                                  & 0.1489788             & \cellcolor[HTML]{F2F2F2}\textbf{0.1477036} & 0.1477758              & 0.1480055              & 0.1482378              & 0.148935                \\ \bottomrule
    \end{tabular}
\end{table*}







\begin{table*}[!ht]
    \centering
    \caption{Hyperparameter sensitivity analysis of the VE pipeline with respect to the variate embedding dimension ($k$) and parameter size expansion factor ($p$) on the Weather dataset. The best results within each parameter size level are shaded, and the absolute \textbf{best result} for each model is highlighted in \textbf{bold}.}
    \label{tab:paramsensitivity}
    \begin{tabular}{@{}ccccccccc@{}}
    \toprule
                                                        &                           & \multicolumn{7}{c}{$k$}                                                                                                                                                                                                                         \\ \cmidrule(l){3-9} 
    \multirow{-2}{*}{Method}                            & \multirow{-2}{*}{$p$}       & 2                                          & 4                                 & 8                                          & 16                                         & 32                                         & 64        & 128       \\ \midrule
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{0.25} & \cellcolor[HTML]{F2F2F2}0.2267947          & 0.228031                          & 0.2296245                                  & 0.2289082                                  & 0.2310323                                  &           &           \\
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{1}    & \cellcolor[HTML]{F2F2F2}0.2226328          & 0.2227887                         & 0.2243922                                  & 0.2257485                                  & 0.2261215                                  & 0.2269735 & 0.2260281 \\
    \multicolumn{1}{c|}{\multirow{-3}{*}{iTransformer}} & \multicolumn{1}{c|}{4}    & 0.2228577                                  & 0.2199955                         & \cellcolor[HTML]{F2F2F2}\textbf{0.2195231} & 0.2214849                                  & 0.222228                                   & 0.2249379 & 0.2246715 \\ \midrule
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{0.25} & 0.2143703                                  & \cellcolor[HTML]{F2F2F2}0.211337  & 0.2181442                                  & 0.223941                                   &                                            &           &           \\
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{1}    & 0.2075411                                  & \cellcolor[HTML]{F2F2F2}0.2012737 & 0.2030463                                  & 0.2064978                                  & 0.2097026                                  & 0.2118939 &           \\
    \multicolumn{1}{c|}{\multirow{-3}{*}{Dlinear}}      & \multicolumn{1}{c|}{4}    & 0.2046664                                  & 0.1972951                         & \cellcolor[HTML]{F2F2F2}\textbf{0.1964375} & 0.1965331                                  & 0.198918                                   & 0.2018006 & 0.2053406 \\ \midrule
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{0.25} & 0.2063784                                  & \cellcolor[HTML]{F2F2F2}0.2018921 & 0.2071244                                  & 0.212573                                   &                                            &           &           \\
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{1}    & 0.2002722                                  & \cellcolor[HTML]{F2F2F2}0.1931964 & 0.1939487                                  & 0.1952246                                  & 0.1982629                                  & 0.2039194 &           \\
    \multicolumn{1}{c|}{\multirow{-3}{*}{Linear}}       & \multicolumn{1}{c|}{4}    & 0.197999                                   & 0.1921374                         & 0.1919117                                  & \cellcolor[HTML]{F2F2F2}\textbf{0.1913762} & 0.19196                                    & 0.1933247 & 0.1949635 \\ \midrule
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{0.25} & \cellcolor[HTML]{F2F2F2}0.194983           & 0.1967256                         & 0.2001208                                  & 0.2023191                                  & 0.2064423                                  &           &           \\
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{1}    & \cellcolor[HTML]{F2F2F2}\textbf{0.1941107} & 0.1963873                         & 0.1968067                                  & 0.20026                                    & 0.1974031                                  & 0.1980518 & 0.200099  \\
    \multicolumn{1}{c|}{\multirow{-3}{*}{PatchTST}}     & \multicolumn{1}{c|}{4}    & \cellcolor[HTML]{F2F2F2}0.1949145          & 0.1958939                         & 0.195652                                   & 0.1973398                                  & 0.1957348                                  & 0.1959685 & 0.197559  \\ \midrule
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{0.25} & 0.1924287                                  & 0.1899614                         & \cellcolor[HTML]{F2F2F2}0.1875843          &                                            &                                            &           &           \\
    \multicolumn{1}{c|}{}                               & \multicolumn{1}{c|}{1}    & 0.1942909                                  & 0.1874208                         & 0.185515                                   & \cellcolor[HTML]{F2F2F2}\textbf{0.1848733}          & 0.185363                                   &           &           \\
    \multicolumn{1}{c|}{\multirow{-3}{*}{FITS}}         & \multicolumn{1}{c|}{4}    & 0.1946209                                  & 0.1870498                         & 0.1861144                                  & 0.186252                                   & \cellcolor[HTML]{F2F2F2}0.1852288 & 0.18523   & 0.1862641 \\ \bottomrule
    \end{tabular}
\end{table*}












